HRS-Bench: Holistic, Reliable and Scalable Benchmark for Text-to-Image Models

In recent years, Text-to-Image (T2I) models have been extensively studied, especially with the emergence of diffusion models that achieve state-of-the-art results on T2I synthesis tasks. However, existing benchmarks heavily rely on subjective human evaluation, limiting their ability to holistically assess the model's capabilities. Furthermore, there is a significant gap between efforts in developing new T2I architectures and those in evaluation. To address this, we introduce HRS-Bench, a concrete evaluation benchmark for T2I models that is Holistic, Reliable, and Scalable. Unlike existing bench-marks that focus on limited aspects, HRS-Bench measures 13 skills that can be categorized into five major categories: accuracy, robustness, generalization, fairness, and bias. In addition, HRS-Bench covers 50 scenarios, including fashion, animals, transportation, food, and clothes. We evaluate nine recent large-scale T2I models using metrics that cover a wide range of skills. A human evaluation aligned with 95% of our evaluations on average was conducted to probe the effectiveness of HRS-Bench. Our experiments demonstrate that existing models often struggle to generate images with the desired count of objects, visual text, or grounded emotions. We hope that our benchmark help ease future text-to-image generation research. The code and data are available at https://eslambakr.github.io/hrsbench.github.io

==> sections/full_related_work.tex <==
\section{Revisiting Text-to-Image Evaluations}
\label{sec_revisiting_text_to_image_metrics}

% ----------------------------------------------------------------------
\tabcolsep=0.08cm
\begin{table}[t!]
%\captionsetup{font=small}
\centering
\caption{Comparison of various text-to-image benchmarks in terms of: 1) The number of the evaluated models. 2) The number of the covered skills. 3) The number of utilized metrics. 4) The evaluation type, whether human or metric based, or both. 5) The number of prompts. 6) The prompt generation type, whether a template or human-based or both. 7) Whether there are different hardness levels are included. 8) Number of annotators contributed to the evaluation.}


\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{ccccccccccc}
    \toprule[1.5pt]
    \multirow{2}{*}{\textbf{Method}} & \- & \- & \- & \multicolumn{2}{c}{\textbf{Eval Type}} &  \- & \multicolumn{2}{c}{\textbf{Prompt Type}} \\ 
    \- &  \textbf{\# Models} &  \textbf{\# Skills} & \textbf{\# Metrics}  &  \textbf{Human} & \textbf{Auto} & \textbf{\# Prompts} & \textbf{Template} & \textbf{Human} & \makecell{\textbf{Hardness}\\\textbf{Levels}} & \textbf{\# Annotators}\\
   \midrule[0.75pt]
    \textbf{DrawBench} \cite{saharia2022photorealistic} & 5 & 4 & 0 & \cmark & \xmark & 200  & \xmark & \cmark & \xmark & 25\\
    \textbf{DALL-EVAL} \cite{cho2022dall} & 4 & 5 & 3 & \cmark & \xmark & 7330 & \cmark & \xmark & \xmark & 6\\
    \textbf{HE-T2I} \cite{petsiuk2022human} & 2 & 3 & 0 & \cmark & \xmark & 90 & \xmark & \cmark & \cmark & 20\\
    \textbf{TISE} \cite{dinh2022tise} & 7 & 3 & 5 & \xmark & \cmark & N/A & \xmark & \cmark & \xmark & N/A\\
    \textbf{{\papernameAbbrev} (Ours)} & \textbf{8} & \textbf{13} & \textbf{17} & \textbf{\cmark} & \textbf{\cmark} & \textbf{45000} & \textbf{\cmark} & \textbf{\cmark} & \textbf{\cmark} & \textbf{1000}\\

  \bottomrule[1.5pt]
\end{tabular}
\end{adjustbox}
\label{tab_benchmarks_comparision}
\end{table}
% ----------------------------------------------------------------------

\me{the writing of the related work seems very risky now; will be good to revise all this in a way that acknowledge and appreciate somehow what they did not only discussing the limitations they have}
In recent years, there have been rapid efforts toward designing better image generation models. 
Nonetheless, most \me{it is always risky to say all; instead say most} existing metrics suffer from several limitations that make them far from being reliable; therefore, comparing the existing models is not straightforward and heavily subjective for human evaluations.
Accordingly, in this section, we first dissect the different existing benchmarks, then cover the used metric to evaluate text-to-image models, showing their shortcomings. 
Motivated by their limitations\me{3-4 times in same paragraph mentioning the word limitation; a bit too much}, which raises many questions, we take one step toward designing a more holistic, robust and reliable benchmark, termed {\papernameAbbrev}\me{this statement is good, focus more on the significant steps you are making}, discussed in Section \ref{sec_methodology}.

\subsection{Revisiting existing benchmarks}
Table \ref{tab_benchmarks_comparision} summarizes the existing T2I benchmarks.

\noindent --\textbf{DrawBench. \cite{saharia2022photorealistic}} 
As part of Imagen paper, DrawBench is proposed to evaluate the T2I models from other aspects rather than the image quality. 
To this end, DrawBench covers only four basic skills; counting, compositions, conflicting, and writing, by collecting 200 prompts to cover the whole skills.
Despite the simplicity and the limited scope of DrawBench, their efforts is appreciated as the first attempt to assess other aspects rather than the image quality.

\noindent --\textbf{DALL-EVAL. \cite{cho2022dall}}
It proposes a toolkit, called PAINTSKILLS, which assesses only three simple visual reasoning skills; object recognition, object counting, and spatial relation understanding, alongside two social bias skills; gender and racial bias.
To facilitate the automatic evaluation, they built a simple unity simulator including limited objects to collect the datasets \me{what makes objects limited; how many compared to yours?}.
DETR \cite{carion2020end} object detector is utilized for visual reasoning skills evaluation after being fine-tuned on the same datasets collect from the simulator.
Despite the efforts done by DALL-EVAL compared to DrawBench \cite{saharia2022photorealistic}, as it is considered as a benchmark paper, in contrast to DrawBench which propose new T2I architecture called Imagen,it is still far away from being holistic benchmark, as only four models are evaluated using only 7k prompts and six annotators. \me{rework the last 1-2 sentences; sentence structure needs to be significantly improved; avoid very long sentences; break it down a bit. Also generally try to avoid passive voice. use more they propose or  we propose. No need to mention DALL-EVAL  is a benchmark paper; mention it once at the beginning of this paragraph that it is a benchmark focused effort in contrast to DrawBench}

\noindent --\textbf{HE-T2I. \cite{petsiuk2022human}}
HE-T2I proposes 32 possible aspects to benchmark T2I models, however, only three of them are explored; counting, shapes, and faces.\me{mention sth positive; don't start with however in the first sentence. say sth positive; the mention the opportunity to improve in contrast }
The three aspects are evaluated using human evaluations, where only twenty annotators have contributed to the evaluation. \me{this is a general issue in the way we cover related work now. please consider when making a pass while discussing all methods}

\noindent --\textbf{TISE. \cite{dinh2022tise}}
TISE introduces a bag of metrics to evaluate T2I models from three aspects; positional alignment, counting, and fidelity. Three fidelity metrics are introduced, i.e., $IS^*$, O-IS, and O-FID, and PA for positional alignment, and CA for counting alignment. 

\subsection{Revisiting  existing T2I metrics}
In addition to the aforementioned benchmarks, other existing work tries to tackle some individual skills: \me{can this be deleted? or say sth more informative like }

\noindent --\textbf{Compositions metrics.}
ComposableDiffusion \cite{liu2022compositional} measure the compositional skill by creating compositions of certain concepts, e.g., composing the language descriptions using the conjunction operator; AND, composing objects' location and objects colors.
To evaluate the object's location and color compositions, CLEVR \cite{johnson2017clevr} and Relational CLEVR \cite{liu2021learning} datasets are utilized and split into training and testing splits. 
Then, the training split is used to train a binary classifier to predict whether the image contains or represents the concept. 
Such a simple metric will fail to measure complex compositions, e.g., language descriptions compositions, therefore, human evaluation only is utilized in this case.
Consequently, StructureDiffusion \cite{feng2022training} introduces two datasets to assess compositionality; Attribute Binding Contrast (ABC-6K) and Concept Conjunction 500 (CC-500). 
ABC-6K consists of 3K contrastive pairs, which are collected by adapting MS-COCO dataset \cite{lin2014microsoft} by switching the position of two colors to create a contrast captions\me{grammer issues in this sentence, can't parse; please fix ``create a contrast captions''?}. 
While CC-500 consists of only 500 template-based prompts, where each prompt contains two objects with two different colors.
Nevertheless, these two datasets \cite{feng2022training} are not sufficient for holistic evaluation of the compositional skill due to their simplicity.
In addition, their automatic evaluation metric; GLIP \cite{li2022grounded}, shows a low consistency rate with humans; around 48\%.
CLIP-R-Precision \cite{park2021benchmark} assesses text-to-image alignment for novel compositions, and proposes any metric \me{propose any metric? can't undertsand}, termed CLIP-R-Precision, based on CLIP.
However, Winoground \cite{thrush2022winoground} and ARO \cite{yuksekgonul2022and} show the deficiency of large pre-trained models, e.g., CLIP, in compositional understanding.

\noindent --\textbf{Bias metrics.}
GEP \cite{zhang2023auditing} studies how gender is presented differently in text-to-image models by probing gender indicators in the input text.
Additionally, an automatic metric, termed GEP, is introduced to measure gender presentation differences.\me{how?. are you doing it differently}

\noindent --\textbf{Fidelity metrics.} 
To evaluate fidelity, two common metrics have been widely used: Inception score (IS)~\cite{NIPS2016_8a3363ab} and Fréchet Inception Distance (FID)~\cite{NIPS2017_8a1d6947}. 
The Inception Score measures the quality and diversity of generated images~\cite{NIPS2016_8a3363ab}. A higher score indicates better image quality and diversity. 
The Fréchet Inception Distance measures the distance between the distribution of real images and generated images in feature space~\cite{NIPS2017_8a1d6947}. A lower FID score indicates a closer match between the distributions and therefore better image quality. 

While these metrics are commonly used, FID has been shown highly biased~\cite{fidbias} and IS does not take intra-class diversity into account~\cite{isbad} and suffers from inconsistency~\cite{is_incon}. 
Both FID and IS lack robustness~\cite{fid_is_rob}. 
FID and Inception Score are objective metrics that rely on predefined criteria for image quality. However, human perception of image quality is subjective and may vary depending on individual preferences and context. To ensure a fair comparison of different models for fidelity, we, therefore, use only human evaluations to rank the models.

\me{However, IS does not measure the diversity of the generation compared to real data and can be hacked to produce a high score if the model generates one example from every class. Say also that it is dependent on the inception model and hence is generated objects are outside that scope; the measure will be less and less accurate; and also say if thee intent is to use to model to product out of domain images or sth novel. It will not be the right metric; argue why}

